Measuring Robustness in Cyber-Physical Systems under Sensor Attacks

This paper contributes a formal framework for quantitative analysis of bounded sensor attacks on cyber-physical systems, using the formalism of differential dynamic logic. Given a precondition and postcondition of a system, we formalize two quantitative safety notions, quantitative forward and backward safety, which respectively express (1) how strong the strongest postcondition of the system is with respect to the specified postcondition, and (2) how strong the specified precondition is with respect to the weakest precondition of the system needed to ensure the specified postcondition holds. We introduce two notions, forward and backward robustness, to characterize the robustness of a system against sensor attacks as the loss of safety. To reason about robustness, we introduce two simulation distances, forward and backward simulation distances, which are defined based on the behavioral distances between the original system and the system with compromised sensors. Forward and backward distances, respectively, characterize upper bounds of the degree of forward and backward safety loss caused by the sensor attacks. We verify the two simulation distances by expressing them as modalities, i.e., formulas of differential dynamic logic, and develop an ad-hoc proof system to reason with such formulas. We showcase our formal notions and reasoning techniques on two non-trivial case studies: an autonomous vehicle that needs to avoid collision and a water tank system.

==> proof.rules.tex <==

\section{Proof Systems for Reasoning with Simulation Distances} \label{sec:proving-h-eq}


The modality-based encoding described in the previous section is very intuitive, but it may be difficult to reason with. In this section, we introduce two sets of proof rules to reasoning with, respectively, forward and backward distances. We elaborate on both in detail.  

\subsection{Proof System for Forward Distance}


We first introduce the proof rules for forward distance, distinguishing between rules to deal with the cyber components of a CPS, given in Table~\ref{fig:forward-robustness-rules}, and rules to deal with 
physical components expressed in terms of ODEs, and detailed  Table~\ref{fig:forward-robustness-rules-ODE}. 
We start with the first set. 

 In general, the rules build on a judgement that is a generalization of the definition of forward distance. In particular, we write $\FjdmtH{\DLfmlsym}{\DLfmlsymp}{\Pwoattack}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}$ to state that, for each state $\statesymp_1 \in \dLfmlsemstate{\SP{\Qattacked{\Pwoattack}{\sensorset}{\offsetsym}}{\DLfmlsymp}}$ there exists a state $\statesymp_2 \in \dLfmlsemstate{\SP{\Pwoattack}{\DLfmlsym}} $ such that $\Hdiststate{\statesymp_1}{\statesymp_2}{\Hsymbol} \le \Hdistdegsym$. 
%%%
Intuitively, for any execution of the compromised program under precondition $\DLfmlsymp$ there is an execution of the genuine program under precondition $\DLfmlsym$  such that the distance between the corresponding final states is bound by $\Hdistdegsym$. 
%%%
The judgement collides with the definition of forward distance when precondition $\DLfmlsym$ and $\DLfmlsymp$ collapse. We also write $\simuSetH{\DLfmlsymp}{\DLfmlsym}{\Hdistdegsym}{\Hsymbol}$ to mean that for each state $\statesymp_1 \in \DLsem{\DLfmlsymp}$ there exists a state $\statesymp_2 \in  \DLsem{\DLfmlsym}$ such that $\Hdiststate{\statesymp_1}{\statesymp_2}{\Hsymbol} \le \Hdistdegsym$. 



\begin{comment}
\newcommand{\DLfmlsymtest}{\DLfmlsym_t}

\newcommand{\DLfmlsymInv}{\DLfmlsym_i}

\newcommand{\Hdistdegsymp}{\Hdistdegsym_1}
\end{comment}

\begin{table}[H]
  \begin{mathpar}
  
    \inferrule[f-def]
    {     \simuSetH{\SP{\Qattacked{\Pwoattack}{\sensorset}{\offsetsym}}{\DLfmlsymp}}{\SP{\Pwoattack}{\DLfmlsym}}{\Hdistdegsym}{\Hsymbol}
    }
    { \FjdmtH{\DLfmlsym}{\DLfmlsymp}{\Pwoattack}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}      
    }

     \inferrule[f-weaken-l]
    {
      \FjdmtH{\DLfmlsym}{\DLfmlsymp}{\Pwoattack}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol} \\
      \DLfmlsym \rightarrow \DLfmlsym^\prime
    }
    { \FjdmtH{\DLfmlsym^\prime}{\DLfmlsymp}{\Pwoattack}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}   
    }


    
     \inferrule[f-weaken-r]
    {
      \FjdmtH{\DLfmlsym}{\DLfmlsymp}{\Pwoattack}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol} \\
      \DLfmlsymp^\prime \rightarrow \DLfmlsymp
    }
    { \FjdmtH{\DLfmlsym}{\DLfmlsymp^\prime}{\Pwoattack}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}   
    }

  
        
     \inferrule[f-weaken-H]
    {
      \FjdmtH{\DLfmlsym}{\DLfmlsymp}{\Pwoattack}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol} \\
      \DLvarsym \in \Hsymbol 
    }
    { \FjdmtH{\DLfmlsym}{\DLfmlsymp}{\Pwoattack}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol$\setminus 
     \{x\}$}   
    }
    





    
    \inferrule[f-sequence]
    {
      \FjdmtH{\DLfmlsymb}{\DLfmlsympb}{\DLprogsymp}{\sensorset}{\offsetsym}{\Hdistdegsym}{$\Hsymbol$} \\
      \DLfmlsymb = \SP{\DLprogsym}{\DLfmlsyma} \\
      \DLfmlsympb = \SP{\Qattacked{\DLprogsym}{\sensorset}{\offsetsym}}{\DLfmlsympa} 
    }
    { \FjdmtH{\DLfmlsyma}{\DLfmlsympa}{\DLseq{\DLprogsym}{\DLprogsymp}}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}      
    }

    \inferrule[f-choice]
    {
      \FjdmtH{\DLfmlsym}{\DLfmlsymp}{\DLprogsym}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol} \\
      \FjdmtH{\DLfmlsym}{\DLfmlsymp}{\DLprogsymp}{\sensorset}{\offsetsym}{\Hdistdegsymp}{\Hsymbol}
    }
    {
      \FjdmtH{\DLfmlsym}{\DLfmlsymp}{\DLchoice{\DLprogsym}{\DLprogsymp}}{\sensorset}{\offsetsym}{\max(\Hdistdegsym, \Hdistdegsymp)}{\Hsymbol}      
    }
    
    \inferrule[f-test]
    { \simuSetH{ (\DLfmlsymtest \land \DLfmlsymp) }{ (\DLfmlsymtest \land \DLfmlsym) }{\Hdistdegsym}{\Hsymbol}
    }
    {      \FjdmtH{\DLfmlsym}{\DLfmlsymp}{\DLtest{\DLfmlsymtest}}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}      
    }

    
    \inferrule[f-dassign]
    {
      \simuSetH{\DLfmlsymp}{\DLfmlsym}{\Hdistdegsym}{\Hsymbol} \\
      \DLvarsym \not\in \Hsymbol
    }
    {
      \FjdmtH{\DLfmlsym}{\DLfmlsymp}{\DLassign{\DLvarsym}{\DLtermsym}}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}      
    }
    

    
    \inferrule[f-dassign-read]
    {
      \simuSetH{\DLfmlsymp}{\DLfmlsym}{\Hdistdegsym}{\Hsymbol} \\
      q_{s} \in \sensorset \\     q_{s},q_{p} \in\Hsymbol
    }
    {
      \FjdmtH{\DLfmlsym}{\DLfmlsymp}{\DLassign{q_{s}}{q_{p}}}{\sensorset}{\offsetsym}{\sqrt{2} \cdot \Hdistdegsym+\offsetsym(q_s)} {\Hsymbol}      
    }
    




    \inferrule[f-nassign]
    { \simuSetH{\DLfmlsymp}{\DLfmlsym}{\Hdistdegsym}{\Hsymbol$\setminus \{x\}$}
    }
    {      \FjdmtH{\DLfmlsym}{\DLfmlsymp}{\DLassignN{\DLvarsym}}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}      
    }
    

    % {
    % \inferrule[f-loop-invariant\text{\color{red}(do we need this rule?)} ]
    % {
    %   \simuSetH{\DLfmlsymp}{\DLfmlsym}{\Hdistdegsym}{\Hsymbol}\\
    %   \DLfmlsym \rightarrow \WP{\DLprogsym}{\DLfmlsym} \text{\color{red}(This doesn't matter)} \\
    %   \DLfmlsymp \rightarrow \WP{\Qattacked{\DLprogsym}{\sensorset}{\offsetsym}}{\DLfmlsymp} 
    % }
    % {     \FjdmtH{\DLfmlsym}{\DLfmlsymp}{\DLloop{\DLprogsym}}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}
    % }
    % }

   
    \inferrule[f-loop]
    {
      \simuSetH{\DLfmlsymp}{\DLfmlsym}{\Hdistdegsym}{\Hsymbol}\\
    %  \DLfmlsym \rightarrow \SP{\DLloop{\DLprogsym}}{\DLfmlsym} \\
      \DLfmlsymp \rightarrow \WP{\Qattacked{{\DLprogsym}}{\sensorset}{\offsetsym}}{\DLfmlsymp} 
    }
    {     \FjdmtH{\DLfmlsym}{\DLfmlsymp}{\DLloop{\DLprogsym}}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}
    }


    \\\\

\inferrule[f-loop-rel-inv]
      {
        \renaming{\DLfmlsym}{\renamingsym}  \land \DLfmlsymp \rightarrow \DLfmlsymInv \\
        \DLfmlsymInv  \rightarrow \WP{\DLseq{\renaming{\Pwoattack}{\renamingsym}}{\Qattacked{\Pwoattack}{\sensorset}{\offsetsym}}}
        {
          \DLfmlsymInv
        } \\
        \DLfmlsymInv \rightarrow (\HdistRenaming{\Hsymbol}{\renamingsym} \leq \Hdistdegsym)
      }
      {     
        \FjdmtH{\DLfmlsym}{\DLfmlsymp}{\DLloop{\Pwoattack}}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}
      }
      \\\\
    
   
     {\color{red}
      \inferrule[f-loop-mono-new]
      {
        \simuSetH{\DLfmlsymp}{\DLfmlsym}{\Hdistdegsym}{\Hsymbol}\\
        \WP{\DLseq{\renaming{\Ps}{\renamingsym}}{\Qattacked{\Ps}{\sensorset}{\offsetsym}}}
        {
          ((\HdistRenaming{\Hsymbol}{\renamingsym})^\prime \leq 0)
        }
      }
      {     
        \FjdmtH{\DLfmlsym}{\DLfmlsymp}{\DLloop{\Ps}}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}
      }
      }

      \\\\

      {\color{red}
    \inferrule[f-loop-mono]
    {
      \simuSetH{\DLfmlsymp}{\DLfmlsym}{\Hdistdegsym}{\Hsymbol}\\
      \DLfmlsym \land \renaming{\DLfmlsymp}{\renamingsym}  \rightarrow \DLfmlsymInv \\
      \DLfmlsymInv  \rightarrow \WP{\DLseq{\renaming{\DLprogsym}{\renamingsym}}{\Qattacked{\DLprogsym}{\sensorset}{\offsetsym}}}
      {
        \DLfmlsymInv
      } \\
      \DLfmlsymInv \rightarrow ((\HdistRenaming{\Hsymbol}{\renamingsym})^\prime \leq 0)
    }
    {     \FjdmtH{\DLfmlsym}{\DLfmlsymp}{\DLloop{\DLprogsym}}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}
    }
    }
    
    % \inferrule[f-ODE-const]
    % {
    %   \simuSetH{\DLfmlsymp}{\DLfmlsym}{\Hdistdegsym}{\Hsymbol}
    % }
    % { \FjdmtH{\DLfmlsym}{\DLfmlsymp}{\dLODE{\DLvarsym}{\DLconst}}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}      
    % }
  \end{mathpar}
  \caption{Proof system for forward distance to deal with cyber components}
  \label{fig:forward-robustness-rules}
\end{table}          

%
Rule \textsc{f-def} is defined based on the definition of the judgement. This rule can be applied on every program construct as long as we can compute the strongest postcondition for that construct. 
%
Rule \textsc{f-weaken-l} is sound since starting from a weaker precondition for the original program we can obviously reach more states. Thus, the forward distance won't increase.
%
Rule \textsc{f-weaken-r} is sound since a stronger precondition of the compromised program means that it can reach less states. Again, the forward distance won't increase.
%
Rule \textsc{f-weaken-h} is sound since the distance with respect to $\Hsymbol \setminus \{x\}$ is not greater than the distance with respect to $\Hsymbol$.
%
\looseness=-1

Rule \textsc{f-sequence} follows the semantics of forward simulation, and decomposes the reasoning of forward distance for a composed program into reasoning of forward distance for two subprograms.
%
Rule \textsc{f-choice} is sound because the maximum value of $\Hdistdegsym$ and $\Hdistdegsymp$ must be a valid forward distance for nondeterministic choice between the two subprograms. 
%
Rule \textsc{f-test} follows the semantics of test of formulas. 
%
For deterministic assignments, Rule \textsc{f-dassign} is sound since the forward distance won't increase if the variable being assigned doesn't belong to the set $\Hsymbol$.
%
Rule \textsc{f-nassign} specifies the forward distance with respect to $\Hsymbol\! \setminus\! \{x\}$ would also be the forward distance for the nondeterministic assignment, as the execution of the genuine program that begins with $\DLfmlsym$ can always pick the same value for $\DLvarsym$ as the execution of compromised one that begins with $\DLfmlsymp$. 
%
Rule \textsc{f-loop} is sound because \DLfmlsymp is an invariant of the compromised program, and thus any reachable states of the compromised program would satisfy $\DLfmlsymp$. We can then always find a reachable state of the genuine program, e.g., $\DLloop{\DLprogsym}$, where the forward distance holds. 


Rule \textsc{f-loop-mono} %%% is a special rule. It 
builds on a relational invariant $\DLfmlsymInv$ between the compromised and genuine programs. Intuitively, the rule says the forward distance between the compromised and genuine programs doesn't increase, if the derivative of the distance is non-increasing as the loop iterates. We elaborate the detail here. 
% because the \Hsymbol-distance between reachable states of the compromised and genuine programs monotonically decrease as the number of loop iteration increases. We elaborate
%
Note that the compromised and genuine programs often refer to the same set of variables. To express a relational invariant between their executions in one formula, we rename variables used by the genuine program into a fresh set of variables, using a renaming function $\renamingsym$ defined as follows: 
\begin{definition}[Renaming function for \DLprogsym] \label{def:var-rename}  For a \dL program \DLprogsym, a function $\renamingsym : \VAR{\DLprogsym} \rightarrow V$ (where $V$ is a set of variables) is a \emph{renaming function for $\DLprogsym$} if:
  \begin{enumerate}%[noitemsep, topsep=-5pt] 
  \item $\renamingsym$ is a bijection;
  \item For all $x \in \VAR{\DLprogsym}$, $\renamingsym(x) \not\in \VAR{\DLprogsym}$;
  \end{enumerate}
Where function $\VAR{\DLprogsym}$ returns the set of variables accessed by $\DLprogsym$.
\end{definition}
Thus, we write $\renaming{\DLprogsym}{\renamingsym}$ for the program equivalent to $\DLprogsym$ but whose variables have been renamed according to $\renamingsym$. Renaming functions similarly apply to \dL formulas. 
% We also write $\renaming{\traceState}{\renamingsym}$ for the state identical to $\traceState$ but whose domain variables have been renamed according to $\renamingsym$. 

% The exact definitions of variable sets and renaming functions are different for \relDDL and \relLDL. 
% More details about the definitions of variable sets and renaming functions can be found in the Appendix.

% As an example, consider a formula $\relfmlsym$:
% \begin{align*}
%   \relE{(\reltermproj{x}{\lstate} = \reltermproj{x}{\rstate})} \relE{~\rightarrow~} \relfmlModalA{\relprogbi{ \DLassign{y}{x} }{ \DLassign{y}{x} }}{(\reltermproj{y}{\lstate} = \reltermproj{y}{\rstate})}
% \end{align*}
% A renaming function for $\relfmlsym$ is $\renamingsym = \{ \hostE{x} \mapsto \hostE{x_1}, \hostE{y} \mapsto \hostE{y_1} \}$. Then $\renaming{\relfmlsym}{\renamingsym}$ is the following formula:
% \begin{align*}
%   \relE{(\reltermproj{x}{\lstate} = \reltermproj{x_1}{\rstate})} \relE{~\rightarrow~} \relfmlModalA{\relprogbi{ \DLassign{y}{x} }{ \DLassign{y_1}{x_1} }}{(\reltermproj{y}{\lstate} = \reltermproj{y_1}{\rstate})}
% \end{align*}
% Formula $\relfmlsym$ is trivially equivalent to $\renaming{\relfmlsym}{\renamingsym}$.


In Rule \textsc{f-loop-mono}, we have a premise $\DLfmlsymInv \rightarrow ((\HdistRenaming{\Hsymbol}{\renamingsym})^\prime \leq 0)$ to specify that the \Hsymbol-distance is non-increasing as the loop iterates. Here $(\HdistRenaming{\Hsymbol}{\renamingsym})^\prime $ is the derivative of $\HdistRenaming{\Hsymbol}{\renamingsym}$ which is defined as $\sqrt{ \sum_{x \in \Hsymbol} \left(x - \renaming{x}{\renamingsym}\right)^2}$. Intuitively, it computes the \Hsymbol-distance between states of the compromised program and the genuine program (after applying a renaming function $\renamingsym$).  


\begin{example}
Consider again the example of a cooling system where $\DLfmlsym = 99.5 \leq temp_p \land temp_p \leq 101 $ and $\DLfmlsymp = 99.2 \leq temp_p \land temp_p \leq 101.3 $. Let $\Hsymbol$ be $\{ temp_p \}$, then $\simuSetH{\DLfmlsymp}{\DLfmlsym}{\Hdistdegsym}{\Hsymbol}$ for $\Hdistdegsym = 0.3$. Note that $\DLfmlsymp$ is an invariant for the compromised system. Thus, using Rule \textsc{f-loop}, we get a forward distance between the compromised and genuine systems being $0.3$. % By Theorem~\ref{thm:forward_rob} we infer $\Fsafety{\Qattacked{\Pwoattack}{\sensorset}{\offsetsym}}{\dLfmlpre}{\dLfmlpost}{\Qdegsymr}$,  for some  $\Qdegsymr \in [3.7,4]$. 
\end{example}

We can state the soundness of the rules in Table~\ref{fig:forward-robustness-rules}. %with respect the forward simulation distance. 

\textcolor{purple}{Massimo: SIMONE, we agreed to change the formulation in this way}


\begin{lemma}
If  $\FjdmtH{\DLfmlsym}{\DLfmlsymp}{\Pwoattack}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}$  can be derived through rules in Table~\ref{fig:forward-robustness-rules}, then 
for each state $\statesymp_1 \in \dLfmlsemstate{\SP{\Qattacked{\Pwoattack}{\sensorset}{\offsetsym}}{\DLfmlsymp}}$ there exists a state $\statesymp_2 \in \dLfmlsemstate{\SP{\Pwoattack}{\DLfmlsym}} $ such that $\Hdiststate{\statesymp_1}{\statesymp_2}{\Hsymbol} \le \Hdistdegsym$. 
\end{lemma}

When both $\DLfmlsym$ and $\DLfmlsymp$ coincide with precondition $\dLfmlpre$, the rules provide an upper bound to the forward simulation distance. 

\begin{theorem}[Soundness Table~\ref{fig:forward-robustness-rules}]   
\label{th:soundness_proof_rules_forward}
If $\FjdmtH{\dLfmlpre}{\dLfmlpre}{\Pwoattack}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}$ follows from the rules in Table~\ref{fig:forward-robustness-rules}, then 

\[\FHsimulation{\Qattacked{\Pwoattack}{\sensorset}{\offsetsym}}{\Pwoattack}{\dLfmlpre}{\Hsymbol}{\Hdistdegsym} \, . 
\]
%%that is, 
%%for each state $\statesymp_1 \in \dLfmlsemstate{\SP{\Qattacked{\Pwoattack}{\sensorset}{\offsetsym}}{\dLfmlpre}}$ there exists a state $\statesymp_2 \in \dLfmlsemstate{\SP{\Pwoattack}{\dLfmlpre}} $ such that $\Hdiststate{\statesymp_1}{\statesymp_2}{\Hsymbol} \le \Hdistdegsym$. 
\end{theorem}

\smallskip
%%\paragraph{Reasoning with forward distance for ODEs}
ODEs are a crucial part of hybrid programs that model CPSs. 
In Figure~\ref{fig:forward-robustness-rules-ODE}, 
we present four rules to reason with the forward distance for 
the physical components expressed in terms of specific kinds of ODEs. 

\begin{table}[t]
  \begin{mathpar}
  \inferrule[f-ODE-const]
  {
    \simuSetH{\DLfmlsymp}{\DLfmlsym}{\Hdistdegsym}{\Hsymbol}
  }
  { \FjdmtH{\DLfmlsym}{\DLfmlsymp}{\dLODE{\DLvarsym}{\DLconst}}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}      
  }
  \\
  
  \inferrule[f-ODE]
  {
    \simuSetH{\DLfmlsymp}{\DLfmlsym}{\Hdistdegsym}{\Hsymbol}\\  
    \forall t\ge 0 . \,\Hdiststate{f(t)}{g(t)}{\Hsymbol}\le \Hdistdegsymp \\
    \forall  f,g \text{ solutions of } \dLODE{\DLvarsym}{\DLtermsym} 
    \text{ s.t. }  
    f(0)\in \DLsem{\DLfmlsym}, \, g(0)\in \DLsem{\DLfmlsymp}, \,  \Hdiststate{f(0)}{g(0)}{\Hsymbol} \le \Hdistdegsym 
  }
  { \FjdmtH{\DLfmlsym}{\DLfmlsymp}{\dLODE{\DLvarsym}{\DLtermsym}}{\sensorset}{\offsetsym}{ \Hdistdegsymp }{\Hsymbol}      
  }	
  \\


    \inferrule[f-ODE-time]
    {
      \simuSetH{\DLfmlsymp}{\DLfmlsym}{\Hdistdegsym}{\Hsymbol}  \\
      \forall t\in [0,\epsilon].\,\Hdiststate{f(t)}{g(t)}{\Hsymbol}\le  \Hdistdegsymp\\
      \forall  f,g \text{ solutions of } \dLODE{\DLvarsym}{\DLtermsym} 
        \text{ s.t. } 
     f(0)\in \DLsem{\DLfmlsym}, \, g(0)\in \DLsem{\DLfmlsymp}, \,  \Hdiststate{f(0)}{g(0)}{\Hsymbol}\le  \Hdistdegsym \\ 
  }
    { \FjdmtH{\DLfmlsym}{\DLfmlsymp}{\dLODE{\DLvarsym}{\DLtermsym},\,\dLODE{time}{1}\,\&\, time \le \epsilon}{\sensorset}{\offsetsym}{\Hdistdegsymp}{\Hsymbol}      
    }
  \\
  \inferrule[f-ODE-mono]
  {
    \simuSetH{\DLfmlsymp}{\DLfmlsym}{\Hdistdegsym}{\Hsymbol}  \\
    (x-y)(f(x)-f(y)) \leq 0 \text{~(y is a fresh variable for $f$)} \\
  }
  { \FjdmtH{\DLfmlsym}{\DLfmlsymp}{\dLODE{\DLvarsym}{f(x)}}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}      
  }
  
  \end{mathpar}
  \caption{Proof system for  forward distance to deal with physical components}
  \label{fig:forward-robustness-rules-ODE}
  \end{table}  



%
Rule \textsc{f-ODE-const} reasons with ODEs whose derivatives are constant. It is sound because the variables evolve at a constant rate for both the genuine and compromised programs. Thus, the genuine program can maintain its distance to the compromised version no matter what states the compromised version can reach after evolution. 

%  
Rule \textsc{f-ODE} reasons with an ODE whose solutions may be available. Its premises specify that starting from a state in $\DLsem{\DLfmlsym}$ and a state in $\DLsem{\DLfmlsymp}$, which are at most $\Hdistdegsym$ distant, during each (same) passage of time, two solutions of the ODE $\dLODE{\DLvarsym}{\DLtermsym}$ reach states that are at most $\Hdistdegsymp$ distant. 
\textcolor{purple}{Massimo: I have problems in doing the parsing of the previous sentence.}
In other words, for any execution of the ODE that begins with a state in $\DLsem{\DLfmlsymp}$ we can always find an execution of the ODE that begins with a state in $\DLsem{\DLfmlsym}$ that is at most $\Hdistdegsymp$ distant (by evolving for the same amount of duration).  
%
\textcolor{purple}{Massimo: this explanation does not help as $d_1$ comes out of the blue}
Rule \textsc{f-ODE-time} readily extends Rule \textsc{f-ODE} with a clock, using the same insights. 


Rule \textsc{f-ODE-mono} allows to prove that if the derivative of the \Hsymbol-distance is nonincreasing over time for reachable states of two solutions of the ODE, the forward distance for the initial states holds for the ODE. In particular, the premise $(x-y)(f(x)-f(y)) \leq 0$ encodes that the derivative of forward distance between two states are nonincreasing over time. Thus, if $\simuSetH{\DLfmlsymp}{\DLfmlsym}{\Hdistdegsym}{\Hsymbol}$ holds initially, the forward distance \Hdistdegsym always holds for reachable states of the two evolutions after the same duration.


     





\begin{example} Exponential decay is often modeled as $\dLODE{x}{-cx}$ for a \emph{positive} constant $\hostE{c}$. The general solution of this ODE is $x(t) = A*e^{(-ct)}$, and $A=x_0$  corresponds to an initial condition $x_0$.  
%%%%%
For any solution $\sola$ that $\dlsem{\sola(0)}{\DLfmlsym}$, if exists $\statesymp$ such that  $\hostE{\Hdiststate{\sola(0)}{\statesymp}{\Hsymbol} \leq \Hdistdegsym}$, then exists a solution $\solb$ of $\dLODE{x}{-cx}$ such that $\solb(0) = \statesymp$ and $\hostE{\Hdiststate{\sola(t)}{\solb(t)}{\Hsymbol} \leq \Hdistdegsym}$ for all time $t$. That is, the distance between $\sola(t)$ and $\solb(t)$ is nonincreasing along with time $t$.
%%
We can apply Rule \textsc{f-ODE} for such an ODE. In addition, Rule \textsc{f-ODE-mono} also applies since $(x-y)(-cx+cy) = -c(x-y)^2 \leq 0$ holds for a positive $c$. % We can apply Rule \textsc{f-ODE-mono} for such an ODE. 
\end{example}




\begin{theorem}    
\label{th:soundness_proof_rules_forward-ode}
If $\FjdmtH{\DLfmlsym}{\DLfmlsymp}{\Pwoattack}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}$ can be derived through rules in Table~\ref{fig:forward-robustness-rules-ODE}, then for each state $\statesymp_1 \in \dLfmlsemstate{\SP{\Qattacked{\Pwoattack}{\sensorset}{\offsetsym}}{\DLfmlsymp}}$ there exists a state $\statesymp_2 \in \dLfmlsemstate{\SP{\Pwoattack}{\DLfmlsym}} $ such that $\Hdiststate{\statesymp_1}{\statesymp_2}{\Hsymbol} \le \Hdistdegsym$. 
\end{theorem}

% Moreover, in the figure, we can observe that if $A_2$ is greater than $A_1$, the solution $x(t) = A_2*e^{(-ct)}$ should be able to reach all possible values of $x(t) = A_1*e^{(-ct)}$, given enough time. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Proof System for Backward Distance}
As done in the previous subsection, 
we provide the proof rules for backward distance, distinguishing between rules to deal with the cyber components of a CPS, given in Table~\ref{fig:backward-robustness-rules}, and rules to deal with 
physical components expressed in terms of ODEs, and detailed  Table~\ref{fig:backward-robustness-rules-ODE}. 
Again, w start with the first set. 


 The rules use a judgement $\BjdmtH{\DLfmlsym}{\DLfmlsymp}{\Pwoattack}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol} $ to reason with backward distance. The judgement states that, for each state $\statesymp_1 \in \dLfmlsemstate{\DLfmlModalE{\Qattacked{\Pwoattack}{\sensorset}{\offsetsym}}{\DLfmlsymp}}$ there exists a state $\statesymp_2 \in \dLfmlsemstate{\DLfmlModalE{\Pwoattack}{\DLfmlsym}} $ such that $\Hdiststate{\statesymp_1}{\statesymp_2}{\Hsymbol} \le \Hdistdegsym$.
%%%
Intuitively, for any execution of the compromised program satisfying a postcondition $\DLfmlsymp$ there is an execution of the genuine program satisfying the postcondition  $\DLfmlsym$    such that the distance between the corresponding intial states is bound by $\Hdistdegsym$.
%%%
% Here, the value of $\Hdistdegsym$ is an upper bound of the distance in backward simulation, that is, if $\BjdmtH{\DLfmlneg{\dLfmlpost}}{\DLfmlneg{\dLfmlpost}}{\Pwoattack}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}$ and $\BHsimulation{\Qattacked{\Pwoattack}{\sensorset}{\offsetsym}}{\Pwoattack}{\dLfmlpost}{\Hsymbol}{\Hdistdegsym}$, then $\Hdistdegsym \geq \Hdistdegsym$.

\begin{table}[t]
  \begin{mathpar}
   \inferrule[b-def]
    {
      \simuSetH{\DLfmlModalE{\Qattacked{\Pwoattack}{\sensorset}{\offsetsym}}{\DLfmlsymp}}{\DLfmlModalE{\Pwoattack}{\DLfmlsym}}{\Hdistdegsym}{\Hsymbol}
    }
    { \BjdmtH{\DLfmlsym}{\DLfmlsymp}{\Pwoattack}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}      
    }
    
\\

     \inferrule[b-weaken-l]
    {
      \BjdmtH{\DLfmlsym}{\DLfmlsymp}{\Pwoattack}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol} \\
      \DLfmlsym \rightarrow \DLfmlsym^\prime
    }
    { \BjdmtH{\DLfmlsym^\prime}{\DLfmlsymp}{\Pwoattack}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}   
    }
    
     \inferrule[b-weaken-r]
    {
      \BjdmtH{\DLfmlsym}{\DLfmlsymp}{\Pwoattack}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol} \\
      \DLfmlsymp^\prime \rightarrow \DLfmlsymp
    }
    { \BjdmtH{\DLfmlsym}{\DLfmlsymp^\prime}{\Pwoattack}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}   
    }

      {\color{red}
     
        
     \inferrule[b-weaken-H]
    {
      \BjdmtH{\DLfmlsym}{\DLfmlsymp}{\Pwoattack}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol} \\
      \DLvarsym \in \Hsymbol 
    }
    { \BjdmtH{\DLfmlsym}{\DLfmlsymp^\prime}{\Pwoattack}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol$\setminus 
     \{x\}$}   
    }
    }



    
    \inferrule[b-sequence]
    {
      \BjdmtH{\DLfmlsyma}{\DLfmlsympa}{\DLprogsym}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol} \\
      \BjdmtH{\DLfmlsymb}{\DLfmlsympb}{\DLprogsymp}{\sensorset}{\offsetsym}{\Hdistdegsymp}{\Hsymbol} \\
      \DLfmlsyma = \DLfmlModalE{\DLprogsymp}{\DLfmlsymb} \\
      \DLfmlsympa = \DLfmlModalE{\Qattacked{\DLprogsymp}{\sensorset}{\offsetsym}}{\DLfmlsympb} 
    }
    { \BjdmtH{\DLfmlsyma}{\DLfmlsympa}{\DLseq{\DLprogsym}{\DLprogsymp}}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}      
    }

    \inferrule[b-choice]
    {
      \BjdmtH{\DLfmlsym}{\DLfmlsymp}{\DLprogsym}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol} \\
      \BjdmtH{\DLfmlsym}{\DLfmlsymp}{\DLprogsymp}{\sensorset}{\offsetsym}{\Hdistdegsymp}{\Hsymbol}
    }
    {
      \BjdmtH{\DLfmlsym}{\DLfmlsymp}{\DLchoice{\DLprogsym}{\DLprogsymp}}{\sensorset}{\offsetsym}{max(\Hdistdegsym, \Hdistdegsymp)}{\Hsymbol}      
    }

    \inferrule[b-dassign]
    {
      \simuSetH{\DLfmlsymp}{\DLfmlsym}{\Hdistdegsym}{\Hsymbol} \\
      \DLvarsym \not \in \Hsymbol
    }
    {
      \BjdmtH{\DLfmlsym}{\DLfmlsymp}{\DLassign{\DLvarsym}{\DLtermsym}}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}      
    }

    % \inferrule[b-nassign]
    % { \simuSetH{\DLfmlsymp}{\DLfmlsym}{\Hdistdegsym}{\Hsymbol$\setminus\{x\}$}
    % }
    % {      \BjdmtH{\DLfmlsym}{\DLfmlsymp}{\DLassignN{\DLvarsym}}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}     
    % }

    
    {\color{red}
       
    \inferrule[b-dassign-read]
    {
      \simuSetH{\DLfmlsymp}{\DLfmlsym}{\Hdistdegsym}{\Hsymbol} \\
      q_{s} \in \sensorset \\     q_{s},q_{p} \in\Hsymbol
    }
    {
      \BjdmtH{\DLfmlsym}{\DLfmlsymp}{\DLassign{q_{s}}{q_{p}}}{\sensorset}{\offsetsym}{\sqrt{2} \cdot \Hdistdegsym+\offsetsym(q_s)} {\Hsymbol}      
    }
    }
     
    {\color{red}
    \inferrule[b-nassign]
    { \simuSetH{\DLfmlsymp}{\DLfmlsym}{\Hdistdegsym}{\Hsymbol}
    }
    {      \BjdmtH{\DLfmlsym}{\DLfmlsymp}{\DLassignN{\DLvarsym}}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}     
    }
    }

  \inferrule[b-test]
  { \simuSetH{ (\DLfmlsymtest \land \DLfmlsymp) }{ (\DLfmlsymtest \land \DLfmlsym) }{\Hdistdegsym}{\Hsymbol}
  }
  {      \BjdmtH{\DLfmlsym}{\DLfmlsymp}{\DLtest{\DLfmlsymtest}}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}      
  }

    {\color{red} 
    \inferrule[b-loop]
    {
      \simuSetH{\DLfmlsymp}{\DLfmlsym}{\Hdistdegsym}{\Hsymbol}\\
     %  \DLfmlsym \rightarrow \DLfmlModalE{\DLprogsym}{\DLfmlsym} \\
\DLfmlModalE{\Qattacked{\DLprogsym}{\sensorset}{\offsetsym}}{\DLfmlsymp}   \rightarrow \DLfmlsymp 
    }
    {     \BjdmtH{\DLfmlsym}{\DLfmlsymp}{\DLloop{\DLprogsym}}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}         }
    }

% {\color{purple}
%     \inferrule[B-loop-BIS why is this sound?]
% {
% 	\BjdmtH{\DLfmlsym}{\DLfmlsymp}{\DLprogsym}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}\\
% 	{\DLfmlsym}   \rightarrow    \DLfmlsym  \DLfmlModalE{\DLprogsym}{}\\
% 	{\DLfmlsymp}  \rightarrow     \DLfmlsymp\DLfmlModalE{\Qattacked{\DLprogsym}{\sensorset}{\offsetsym}}{} 
% }
% {     \BjdmtH{\DLfmlsym}{\DLfmlsymp}{\DLloop{\DLprogsym}}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}         
% }
% }
  
  {\color{red}
  \inferrule[b-loop-rel-inv]
  {
    \simuSetH{\DLfmlsymp}{\DLfmlsym}{\Hdistdegsym}{\Hsymbol}\\
    \DLfmlsym \land \renaming{\DLfmlsymp}{\renamingsym}  \rightarrow \DLfmlsymInv \\
    \DLfmlModalE{\DLseq{\renaming{\DLprogsym}{\renamingsym}}{\Qattacked{\DLprogsym}{\sensorset}{\offsetsym}}} 
    {
      \DLfmlsymInv
    } \rightarrow  \DLfmlsymInv   \\
    \DLfmlsymInv \rightarrow (\HdistRenaming{\Hsymbol}{\renamingsym} \leq \Hdistdegsym)
  }
  {     \BjdmtH{\DLfmlsym}{\DLfmlsymp}{\DLloop{\DLprogsym}}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}
  }
  }

     {\color{red}
      \inferrule[b-loop-mono-new]
      {
        \simuSetH{\DLfmlsymp}{\DLfmlsym}{\Hdistdegsym}{\Hsymbol}\\
        \WP{\DLseq{\renaming{\DLprogsym}{\renamingsym}}{\Qattacked{\DLprogsym}{\sensorset}{\offsetsym}}}
        {
          ((\HdistRenaming{\Hsymbol}{\renamingsym})^\prime \geq 0)
        }
      }
      {     
        \BjdmtH{\DLfmlsym}{\DLfmlsymp}{\DLloop{\DLprogsym}}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}
      }
    }

  \end{mathpar}
  \caption{Proof rules for backward distance to deal with cyber  components}
  \label{fig:backward-robustness-rules}
\end{table}



%
Rule \textsc{b-def} is defined by the definition of the judgement. This rule can be applied on every program construct so long as we can compute the weakest precondition for that construct. 
%
Rule \textsc{b-weaken-l} is sound since a weakened postcondition for the original program means more possible starting states. The upper bound won't increase.
%
Rule \textsc{b-weaken-r} is sound since a stronger postcondition of the compromised program means less possible starting states. The upper bound won't increase.
%
Rule \textsc{b-sequence} follows the semantics of backward simulation, and decomposes the reasoning of upper bound for a composed program into reasoning of upper bounds for two subprograms.  
%
Rule \textsc{b-choice} is sound because the maximum value of $\Hdistdegsym$ and $\Hdistdegsymp$ must be a backward distance of the nondeterministic choice. 
%
For deterministic assignments, Rule \textsc{b-dassign} is sound since the assignment can only modify the value of variable $\DLvarsym$.
%
Rule \textsc{b-dassign} is sound because the attack cannot compromise or affect the nondeterministic assignment. 
% for any initial state that reaches $\DLfmlsymp$,  we can alway find an initial state of the compromised program that is within  can always choose 
Rule \textsc{b-test} follows the semantics of formula tests. 
%
Rule \textsc{b-loop} is sound because the promise says that the states of $\DLsem{\DLfmlsymp}$ subsume the potential initial states, i.e., $\DLsem{ \DLfmlModalE{\Qattacked{\DLprogsym}{\sensorset}{\offsetsym}}{\DLfmlsymp}}$. And for any state in $\DLsem{\DLfmlsymp}$, we have an initial state in $\DLsem{\DLfmlsym}$ that is at most distance $\Hdistdegsym$. Any states in $\DLsem{\DLfmlsym}$ are also in $\DLsem{ \DLfmlModalE{\DLloop{\DLprogsym}}{\DLfmlsymp}}$. 


\begin{theorem}    
\label{th:soundness_proof_rules_backward}
If $\BjdmtH{\DLfmlsym}{\DLfmlsymp}{\Pwoattack}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}$ can be derived through rules in Table~\ref{fig:backward-robustness-rules}, then for each state $\statesymp_1 \in \dLfmlsemstate{\DLfmlModalE{\Qattacked{\Pwoattack}{\sensorset}{\offsetsym}}{\DLfmlsymp}}$ there exists a state $\statesymp_2 \in \dLfmlsemstate{\DLfmlModalE{\Pwoattack}{\DLfmlsym}} $ such that $\Hdiststate{\statesymp_1}{\statesymp_2}{\Hsymbol} \le \Hdistdegsym$.
\end{theorem}

\smallskip

As we did for forward distance, we present four proof rules, 
given in Table~\ref{fig:backward-robustness-rules-ODE}, 
to reason with backward distance for specific ODEs. 

%
Rule \textsc{b-ODE-const} reasons with ODEs whose derivatives are constant. It is sound because the variables evolve at a constant rate for both the genuine and compromised programs. The distance between potential initial states of the two programs can thus be a constant. 
% Thus, the genuine program can maintain its distance to the compromised version no matter what states the compromised version can reach after evolution. 

%
Rule \textsc{b-ODE} reasons with an ODE whose solutions may be available. It specifies that if two solutions of the ODE $\dLODE{\DLvarsym}{\DLtermsym}$ always reach states that are at most $\Hdistdegsymp$ distant after the same passage of time, their initial states are at most $\Hdistdegsymp$ distant. 
%
Rule \textsc{b-ODE-time} directly extends Rule \textsc{b-ODE} with a clock. 


Rule \textsc{b-ODE-mono} encodes that, intuitively, if the derivative of the \Hsymbol-distance is nondecreasing over time for reachable states of two solutions of the ODE, and the postconditions are at most $\Hdistdegsym$, then the backward distance is at most $\Hdistdegsym$. 


\begin{table}[t]
  \begin{mathpar}
  \inferrule[b-ODE-const]
  {
    \simuSetH{\DLfmlsymp}{\DLfmlsym}{\Hdistdegsym}{\Hsymbol}
  }
  { \BjdmtH{\DLfmlsym}{\DLfmlsymp}{\dLODE{\DLvarsym}{\DLconst}}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}      
  }
  \\
  \inferrule[b-ODE]
  {
    \simuSetH{\DLfmlsymp}{\DLfmlsym}{\Hdistdegsym}{\Hsymbol}\\  
    \forall t\ge 0 . \,\Hdiststate{f(t)}{g(t)}{\Hsymbol}\le \Hdistdegsymp \\
    \forall  f,g \text{ solutions of } \dLODE{\DLvarsym}{\DLtermsym} 
    \text{ s.t. }  
    f(t)\in \DLsem{\DLfmlsym}, \, g(t)\in \DLsem{\DLfmlsymp} 
    , \,  \Hdiststate{f(t)}{g(t)}{\Hsymbol} \le \Hdistdegsym 
  }
  { \BjdmtH{\DLfmlsym}{\DLfmlsymp}{\dLODE{\DLvarsym}{\DLtermsym}}{\sensorset}{\offsetsym}{\Hdistdegsymp}{\Hsymbol}      
  }	
  \\
    \inferrule[b-ODE-time]
    {
      \simuSetH{\DLfmlsymp}{\DLfmlsym}{\Hdistdegsym}{\Hsymbol}  \\
      \forall t\in [0,\epsilon].\,\Hdiststate{f(t)}{g(t)}{\Hsymbol}\le  \Hdistdegsymp\\
      \forall  f,g \text{ solutions of } \dLODE{\DLvarsym}{\DLtermsym} 
        \text{ s.t. } 
     f(t)\in \DLsem{\DLfmlsym}, \, g(t)\in \DLsem{\DLfmlsymp}, \,  
     \Hdiststate{f(t)}{g(t)}{\Hsymbol}\le  \Hdistdegsym \\ 
  }
    { \BjdmtH{\DLfmlsym}{\DLfmlsymp}{\dLODE{\DLvarsym}{\DLtermsym},\,\dLODE{time}{1}\,\&\, time \le \epsilon}{\sensorset}{\offsetsym}{\Hdistdegsymp}{\Hsymbol}      
    }
  \\
  \inferrule[b-ODE-mono]
  {
    \simuSetH{\DLfmlsymp}{\DLfmlsym}{\Hdistdegsym}{\Hsymbol}  \\
    (x-y)(f(x)-f(y)) \geq 0 \text{~(y is a fresh variable for $f$)} \\
  }
  { \BjdmtH{\DLfmlsym}{\DLfmlsymp}{\dLODE{\DLvarsym}{f(x)}}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}      
  }
  
  \end{mathpar}
  \caption{Proof rules for backward distance to deal with physical components}
  \label{fig:backward-robustness-rules-ODE}
  \end{table}  
    


% \paragraph*{Example} 
% Consider the ODE $\dLODE{x}{\omega*y}, \dLODE{y}{-\omega*x}$ for a constant $\hostE{\omega}$. A general solution is $x(t) = A*sin(\omega*t+c),~ y(t) = A*cos(\omega*t+c)$.
% Two solutions of the ODE with different initial conditions would satisfy $\hostE{x^2+y^2 = A^2}$ for different $\hostE{A}$.  \todo{More explanation}

% We know that the solutions are going in circles. Thus, for any point on one circle (one solution), the other solution can reach a point that the distance is $(A1 - A2)$.   

\paragraph*{Example} Exponential growth is often modeled as $\dLODE{x}{cx}$ for a \emph{positive} constant $\hostE{c}$. The general solution of this ODE is $x(t) = A*e^{(ct)}$, and $A=x_0$ corresponds to an initial condition $x_0$.  
%%%%%
For any two solutions $\sola$ and $\solb$, we know that if $\hostE{\Hdiststate{\sola(t')}{\solb(t')}{\Hsymbol} = \Hdistdegsym}$ for some $t'$, then $\hostE{\Hdiststate{\sola(t)}{\solb(t)}{\Hsymbol} \leq \Hdistdegsym}$ for all time $t \le t'$. That is, the distance between $\sola(t)$ and $\solb(t)$ is non-decreasing over time $t$.
% $\sola$ that $\dlsem{\sola(t)}{\DLfmlsym}$, if exists $\statesymp$ that  $\hostE{\Hdiststate{\sola(t)}{\statesymp}{\Hsymbol} \leq \Hdistdegsym}$, then exists a solution $\solb$ of $\dLODE{x}{cx}$ that $\solb(t) = \statesymp$ and $\hostE{\Hdiststate{\sola(t)}{\solb(t)}{\Hsymbol} \leq \Hdistdegsym}$ for all time $t \ge 0$. That is, the distance between $\sola(t)$ and $\solb(t)$ is non-decreasing along with time $t$.
%%
We can apply Rule \textsc{b-ODE-mono} since $(x-y)(cx-cy) = c(x-y)^2 \ge 0$ holds for a positive $c$. % We can apply Rule \textsc{f-ODE-mono} for such an ODE. 


\begin{theorem}    
\label{th:soundness_proof_rules_backward-ode}
If $\BjdmtH{\DLfmlsym}{\DLfmlsymp}{\Pwoattack}{\sensorset}{\offsetsym}{\Hdistdegsym}{\Hsymbol}$ can be derived through rules in Table~\ref{fig:backward-robustness-rules-ODE}, then for each state $\statesymp_1 \in \dLfmlsemstate{\DLfmlModalE{\Qattacked{\Pwoattack}{\sensorset}{\offsetsym}}{\DLfmlsymp}}$ there exists a state $\statesymp_2 \in \dLfmlsemstate{\DLfmlModalE{\Pwoattack}{\DLfmlsym}} $ such that $\Hdiststate{\statesymp_1}{\statesymp_2}{\Hsymbol} \le \Hdistdegsym$.
\end{theorem}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

